Dissecting Android Cryptocurrency Miners

Cryptojacking applications pose a serious threat to mobile devices. Due to the extensive computations, they deplete the battery fast and can even damage the device. In this work we make a step towards combating this threat. We collected and manually verified a large dataset of Android mining apps. In this paper, we analyze the gathered miners and identify how they work, what are the most popular libraries and APIs used to facilitate their development, and what static features are typical for this class of applications. Further, we analyzed our dataset using VirusTotal. The majority of our samples is considered malicious by at least one VirusTotal scanner, but 16 apps are not detected by any engine; and at least 5 apks were not seen previously by the service. Mining code could be obfuscated or fetched at runtime, and there are many confusing miner-related apps that actually do not mine. Thus, static features alone are not sufficient for miner detection. We have collected a feature set of dynamic metrics both for miners and unrelated benign apps, and built a machine learning-based tool for dynamic detection. Our BrenntDroid tool is able to detect miners with 95% of accuracy on our dataset. This preprint is a technical report accompanying the paper "Dissecting Android Cryptocurrency Miners" published in ACM CODASPY 2020.

==> sections/economics.tex <==

\section{Economics of Mining}
\OG{Here I put some initial ideas and references}

\subsection{Cryptojacking}

\begin{table*}
\scriptsize
%\lessspace
%\renewcommand{\arraystretch}{1.5}
\centering
\caption{Cryptojacking: What is where}
\begin{tabular}{m{2.2cm} | C{1.4cm} C{2.2cm} C{1cm} C{1.2cm} C{1.4cm} C{1.2cm} C{1.2cm} C{2cm}}
\hline
\textbf{Paper} & \textbf{Platform} & \textbf{Currencies} & \textbf{Hash rate} & \textbf{Campaigns} & \textbf{Profits for attacker} & \textbf{Costs for attacker} & \textbf{Costs for user} & \textbf{Other economics} \\ 
\hline
Konoth et al.~\cite{konoth2018minesweeper} & Browser/ Web & Monero/CH & $\checkmark$ & $\checkmark$  & $\checkmark$ &  & & throttling \\
Ruth et al.~\cite{ruth2018digging} & Browser/ Web & Monero/CH & & & $\checkmark$ & & & short links of CH\\
Musch et al.~\cite{musch2018web} & Browser/ Web & Monero, Electroneum, Bytecoin, Intense Coin, Graffiti Coin & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & throttling \\
Saad et al.~\cite{saad2018end} &Browser/ Web & Monero/CH, JSEcoin & $\checkmark$ & & $\checkmark$ & &  $\checkmark$ & feasibility analysis of cryptomining, incl. cost/benefit and throttling\\
Hong et al.~\cite{hong2018you} & Browser/ Web & only list of mining services. & & &$\checkmark$ & & $\checkmark$  &mining participants analysis\\
Pastrana and Suarez-Tangil~\cite{pastrana2019first} & PC/ Binary & Monero, Bitcoin, zCash, Ethereum, Electroneum and others. & & $\checkmark$ & $\checkmark$ & & & underground markets analysis\\
Clay, Hargrave and Sridhar~\cite{clay2018power} & Mobile/ Web & Monero/CH &  & & & & $\checkmark$ & \\
Papadopoulos, Ilia and Markatos~\cite{papadopoulos2018truth} & Browser/ Web & Monero, JSEcoin & $\checkmark$ & & $\checkmark$ & & $\checkmark$ & comparison to profitability from ads \\
Huang et al.~\cite{huang2014botcoin} & PC/ Binary & Bitcoin, Litecoin & $\checkmark$ & $\checkmark$ & $\checkmark$ & & & botnet profits analysis \\

%reference~\cite{} & & & & & & & & \\
\hline
\end{tabular}
\label{tab:summary_soa_economics}
\end{table*}

%\paragraph{Cryptomining technologies/platforms investigated}

\paragraph{Device hash rates given in papers}
Konoth et al.~\cite{konoth2018minesweeper} have estimated hash rates for Coinhive-based in-browser mining for several types of devices: smartphones from lower-end to high-end, intel i3 laptop and intel i7 desktop. 

Musch et al.~\cite{musch2018web} have estimated hash rates for several devices (3 intel i7 devices, intel xeon e5, iphone 8+, a huawei smartphone).

Saad et al.~\cite{saad2018end} have reported on hash rates for 3 systems: windows, linux and Android-based, including with throttling.

Papadopoulos, Ilia and Markatos~\cite{papadopoulos2018truth} reported hash rates for a desktop with intel i7 running in 4 modes.

Huang et al.~\cite{huang2014botcoin} have suggested some hash rates for low-, medium- and high-end PCs (for Bitcoin mining).

\paragraph{Campaigns}
Konoth et al.~\cite{konoth2018minesweeper} have identified 11 campaigns as unique combinations of site keys and WebSocket proxy servers, and 9 campaigns based on proxy-only. For the campaigns, they have computed the number of participating websites. Campaigns have been clustered as 1) third-party website campaigns, 2) ad-based, 3) hacked websites, and 4) torrent portals.   

Musch et al.~\cite{musch2018web} have clustered websites in their sample based on site keys and wallets addresses.

Hong et al.~\cite{hong2018you} have grouped attackers based on wallet addresses.

Pastrana and Suarez-Tangil~\cite{pastrana2019first} have identified campaigns based on several features: same id (wallet, email, etc.), same ancillary files, same hosting server, known mining campaign, domain aliases, mining proxies. They have identified 11,887 campaigns.



\paragraph{Profits for the attacker/mining host}
Konoth et al.~\cite{konoth2018minesweeper} estimated cryptomining profits based on hash rates and the estimated the number of users per month on each website (collecting statistics of the user devices and time spent on website from SimilarWeb). MineCryptoNite provides an API to estimate the mining reward based on these data. Profits have been estimated per campaign and per website.

Musch et al.~\cite{musch2018web} have estimated an upper-bound of profits for a website hosting CoihHive miner based on the Pornhub website usage (number of users and time spent), and have reported on expected revenues for 10 most profitable websites in their sample, and an average profit per mining website. They have also investigated the balances maintained by pools for wallets in their dataset, estimating the cash flow across these wallets at the time of writing.

Ruth et al.~\cite{ruth2018digging} have evaluated the total income of the CoinHive based on the estimated difficulty of PoWs and hence hash rate of the whole network. They reported that, based on their estimations, mining could not be a viable alternative to ads.

Saad et al.~\cite{saad2018end} have estimated profits of a browser-based miner on one battery charge, and have evaluated cryptomining as a bad alternative to ads (i.e., ads bring more profits to websites). They have also estimated monthly profits for the top-10 websites in their sample.

Hong et al.~\cite{hong2018you} have estimated website profits from cryptomining using the number of user and duration of website visit statistics, and an average CPU power/hash rate estimation, difficulty and reward (all three from the CoinHive statistics).

Pastrana and Suarez-Tangil~\cite{pastrana2019first} have evaluated profits for Monero campaigns in their sample, using data published by mining pools (for the wallets from their sample, when available). They provide results for earning estimation for top 10 campaigns from their Monero sample, and a bit more detailed historical analysis of earnings for two largest campaigns.

Papadopoulos, Ilia and Markatos~\cite{papadopoulos2018truth} have simulated mining profits for a website that 100,000 users visit for 1 minute. They evaluated that such a website needs to keep users engaged for much longer time in order to get revenues comparable to ads.

Huang et al.~\cite{huang2014botcoin} have analysed Bitcoin mining malware and estimated earnings of botnets. They have proposed a formula to compute mining revenue as revenue = time of mining $\times$ combined hash rate of botnet $\times$  expected profitability per hash rate $\times$ exchange rate of cryptocurrency.

\paragraph{Costs for the attacker}

Huang et al.~\cite{huang2014botcoin} have considered the costs of bot acquisition and the monetization scheme costs as components of the cost structure for the bot master (attacker). Their analysis suggests that in 2012 -- Q1 2013 Bitcoin miner in botnets was profitable. There were botnets dedicated only to bitcoin mining. After that period, the profits have been less clear. The authors note that the marginal cost of adding mining to already existing botnet is very low, and it is their conclusion that the costs of software development and management costs associated with illicit Bitcoin mining can benefit from the economies of scale. They thus conclude that they expect Bitcoin mining to remain at least marginally profitable for large botnets. 

\paragraph{Costs for the user}
Saad et al.~\cite{saad2018end} have used battery drain and electricity costs as an estimate for user costs.

Hong et al.~\cite{hong2018you} have estimated the combined energy consumption based on the user statistics (as used for computing profits) for their sample websites.

Clay, Hargrave and Sridhar~\cite{clay2018power} have analysed the power consumption of a CoinHive script running in several modes on a Samsung Galaxy S4 device, compared to battery consumption of websites (Amazon and The Guardian pages), and average power consumption without browsing or mining activity.

Papadopoulos, Ilia and Markatos~\cite{papadopoulos2018truth} have estimated the costs imposed on a website user in terms of CPU and memory consumption, network activity (also projecting monetary costs), energy consumption and system temperature profiles, in comparison to in-browser ads.

\paragraph{Other useful info and data sources}
Konoth et al.~\cite{konoth2018minesweeper} have evaluated hash rates and potential profits considering different throttling settings. They also mentioned statistics about observed throttling behavior in websites.

Musch et al.~\cite{musch2018web} have reported on the throttling behavior in their sample.

Ruth et al.~\cite{ruth2018digging} have analysed the short link system provided by CoinHive (users 'pay' for the short link by doing some hashing first). 

Hong et al.~\cite{hong2018you} have reported on the mining process agents (deployers, distributors, pools) and their prevalence and lifecycle in the observed sub-sample. 

Pastrana and Suarez-Tangil~\cite{pastrana2019first} have performed analysis of posts in underground markets to explore malicious miner economy (what is offered, how binaries are monetised, what posts are about).

\subsection{Economic models for cryptomining}
Altman et al.\cite{altman2018mining} have modeled mining competitions and multi-cryptocurrency ecosystem in the game-theoretic way.

